Order out of Chaos: Proving Linearizability Using Local Views

Proving the linearizability of highly concurrent data structures, such as those using optimistic concurrency control, is a challenging task. The main difficulty is in reasoning about the view of the memory obtained by the threads, because as they execute, threads observe different fragments of memory from different points in time. Until today, every linearizability proof has tackled this challenge from scratch. We present a unifying proof argument for the correctness of unsynchronized traversals, and apply it to prove the linearizability of several highly concurrent search data structures, including an optimistic self-balancing binary search tree, the Lazy List and a lock-free skip list. Our framework harnesses {\em sequential reasoning} about the view of a thread, considering the thread as if it traverses the data structure without interference from other operations. Our key contribution is showing that properties of reachability along search paths can be deduced for concurrent traversals from such interference-free traversals, when certain intuitive conditions are met. Basing the correctness of traversals on such \emph{local view arguments} greatly simplifies linearizability proofs. To apply our framework, the user proves that the data structure satisfies two conditions: (1) acyclicity of the order on memory, even when it is considered across intermediate memory states, and (2) preservation of search paths to locations modified by interfering writes. Establishing the conditions, as well as the full linearizability proof utilizing our proof argument, reduces to simple concurrent reasoning. The result is a clear and comprehensible correctness proof, and elucidates common patterns underlying several existing data structures.

==> lockfree-list-example-complicated-contains.tex <==
%!TEX root=./main.tex

% \newcommand{\tk}{\code{key}}
% \newcommand{\tn}{\code{ref}}
% \newcommand{\tref}{\code{ref}}
% \newcommand{\tm}{\code{mark}}
% \newcommand{\tmnext}{\code{next}}

% \newcommand{\lflI}[1]{I_{#1}}
% \newcommand{\lflTI}[1]{\delta_{#1}}

% \newcommand{\lflheadobj}{{\tt head}}
% \newcommand{\lfltailobj}{{\tt tail}}

% \newcommand{\lflQReachXYK}[3]{#1\searchpath{#3}{#2}}
% \newcommand{\lflPReachXK}[2]{\diamondminus(\QReachXK{#1}{#2})}
% \newcommand{\lflQReachXK}[2]{\slheadobj\searchpath{#2}{#1}}
% \newcommand{\lflHQReachXK}[3]{\slheadobj\hsearchpath{#3}{#1}#2}
% \newcommand{\lflsearchpath}[1]{\overset{#1}{\leadsto}}
% \newcommand{\lflhsearchpath}[2]{\overset{#1}{\underset{#2}{\leadsto}}}
% \newcommand{\lflnextnode}{\operatorname{nextNode}}

\input{lockfree-list-code}

\section{Example: Lock-Free List-Based Concurrent Set}\label{Se:LockFreeList}

In this section, we apply our approach to verify the lockfree list-based concurrent set algorithm shown in~\Cref{Fi:LFList}.   
The code of the algorithm is based on the algorithm of~\cite[Chapter 9.8]{TAOMPP},  adapted to our language.
The algorithm is explained in detail in~\cite{TAOMPP}.
Thus, we only describe the parts necessary to understand our linearizbility proof and the assertions,  written inside curly braces, which annotate the code.

The algorithm uses an underlying sorted
linked-list of dynamically-allocated objects of type \code{LFN}, which we refer to as \emph{nodes}.
Every node has three fields: an integer field {\tk} storing the
key of the node, a pointer field {\tref} pointing to a successor node 
(or to a designated \code{null} value),
and a boolean field {\tm} indicating
that the node was logically deleted from the list. 
The original code~\cite[Figures 9.24 to 9.27]{TAOMPP} is written in Java and keep the {\tref} and {\tm} fields of node using a \emph{markable pointer} (see~\cite[Pragma 9.8.1]{TAOMPP}) to allow reading, writing, and applying CAS to the {\tn} and {\tm} fields
simultaneously.
In our implementation, we encapsulate  these fields inside a pair  comprised of a reference and a boolean field which can be accessed atomically. 
We write \code{x.next.ref} and \code{x.next.mark} to denote accessing the {\tn} and {\tm} fields of the node pointed to by \code{x} separately. We use the notation \code{(succ,marked)}$\leftarrow$\code{x.next},
where \code{succ} is a pointer variable and \code{marked} a boolean variable, 
to denote an atomic assignment of \code{x.next.ref} and \code{x.next.mark} to \code{succ} and \code{marked},
respectively. 
Similarly, we write \code{x.next}$\leftarrow$\code{(succ,marked)} to denote an atomic assignment to the two components of the \code{next} pair of fields of the node pointed to by \code{x}. 
We write \code{CAS(\&x.next,(oldref,oldmark),(newref,newmark))} to denote a \emph{compare and set} operation which atomically reads and writes the {\tref} and {\tm} fields of
the node pointed to by \code{x}. 
We often refer to the pair as the {\tmnext} field of a node.
When the \tm-component of the \code{next} field of a node is set, we say that the field resp. the node are  \emph{marked},
otherwise, we say that they are \emph{unmarked}.



The set algorithm defines four procedures: \code{add},
\code{remove}, and \code{contains}. 
The first who
use the internal \code{find} procedure to traverse the list
and prunes out marked nodes.
In contrast, the \code{contains} method's  traversal of the list is \emph{optimistic}: it is done
without any form of synchronization. As a result,  while a
thread is traversing the list, other threads might concurrently
change the list's structure. 
When verifying this algorithm,  our approach helps in proving that \texttt{contains} is linearizable, 
which is the most difficult part of the proof. 
Proving the linearizability of \code{add} and \code{remove} follows rather easily using invariant-based concurrent reasoning %establishing certain state and transition invariants, 
as discussed below.

\paragraph*{Sentinel nodes and initial states}
The  list has designated sentinel \emph{head} and \emph{tail}
nodes. The \emph{head} node is always pointed to by the shared
variable \code{head} and contains the  value $-\infty$. The
\emph{tail} node is always pointed to by the shared variable
\code{tail}, and contains the  value $\infty$. The value $-\infty$
resp. $\infty$ is smaller resp. greater than any possible value
of a key. When the algorithm starts, it first sets \emph{tail} to be the successor of \emph{head} and sets \emph{tail}'s successor to be \code{null}. The sentinel nodes remain unmarked throughout the execution.

\paragraph*{Verifying invariants using concurrent reasoning}
Procedures \texttt{add}, \texttt{remove}, and \texttt{find}  maintain several  \emph{state} invariants:\footnote{Recall that the \code{contain} does not modify the shared state.}
\begin{compactitem}[]
\item 
($\lflI{rT}$) the tail node is always reachable from the head node, where reachability between nodes is determined in this section by following  $\tref$ fields;
\item 
($\lflI{UB}$) all unmarked nodes are reachable from the \emph{head} node; 
and 
\item 
($\lflI{<}$) if node $v$ is the \tref-successor of node $u$ then the key of $v$ is strictly greater than that of~$u$. 
\end{compactitem}
In addition, the procedures maintains the following   \emph{transition} invariants:
\begin{compactitem}[]
\item 
($\lflTI{k}$) the \code{key} node is immutable; and 
\item
($\lflTI{mn}$) the \code{next} pair of fields become immutable once its \code{mark} component is set to \code{true}.
\end{compactitem}
Verifying the invariants hold is rather straightforward as it merely requires local reasoning about each mutation. 
For example, it is easy to see that the \code{next} field of a marked node is never modified:
The modifications (\Cref{ln:lfn:add-cas,ln:lfn:remove-cas,ln:lfn:find-cas}) are   done using a \code{CAS} operation which may succeed only if the modified \code{next} pair of fields is unmarked. 


\paragraph*{Verifying linearizability}
We prove the linearizability of the algorithm  using an \emph{abstraction function}
$\repfunc: H \totalto \powerset(\mathbb{N})$ that maps a concrete memory state of the list to  the {\em abstract set} represented by this state, and showing that \code{add}  and \code{delete} manipulate this abstraction according to their specification and that .\code{find} does not modify it.
We define $\repfunc$ to map $H$ to the set of keys of the unmarked nodes.
Note that by invariants $\lflI{rT}$, $\lflI{UB}$, and  $\lflI{<}$), these nodes 
are part of the \emph{backbone list}---the sorted list connecting the \emph{head} and \emph{tail} nodes.

\subparagraph*{Verifying linearizability of \code{add} or \code{
remove} }

The proof that  \code{add} or \code{remove}   are linearizable 
follows directly from the invariants once we establish the following properties 
of \code{find}:
(a) it does not change the abstract set represented by the list, and
(b) the pair (\code{pred},\code{curr}) of pointers  is returns is such that the node pointed to by \code{pred} was (i) unmarked and (ii) the \tref-predecessor of the node pointed to by \code{curr} the last time \code{pred.next}  was read.
(Property (b) is required only in the verification of unsuccessful invocations, i.e.,
ones which return \code{false}.)

Note that when \code{find} is invoked to locate a key \code{key}, 
it traverses the list starting from the \emph{head} node until it reaches an unmarked node with a key greater than \code{key}. During the traversal it removes marked nodes (\Cref{ln:lfn:find-snip}) If an attempt to remove a node fails, the procedure restarts.

To verify property (a), we merely need to observe that  \code{find}  removes a marked node \code{curr} by redirecting the \code{ref}-field of its predecessor \code{pred} to point to \code{succ}---\code{curr}'s \code{ref}-successor:
Using compare and swap  (\Cref{ln:lfn:find-snip}) ensures that the updates succeeds only if \code{pred} is unmarked and its \tref-field points to \code{curr}.
The fact that \code{succ} is the \tref-successor of \code{curr} is ensured by transition invariant $\lflTI{mn}$ which prohibit the modification of marked node.
Note that the node pointed to by \code{curr} is guaranteed to be   marked   because after checking its {\tm} field in \Cref{ln:lfn:find-while-mark},   transition invariant $\lflTI{m}$ 
ensures that the node remains marked.

To verify property (b), we note that %we use transition invariant $\lflTI{m}$ again:
after \code{find} traverses a \code{next}-link (\Cref{ln:lfn:find-get-next,ln:lfn:find-get-next-in-while}) it ensures that the node is not marked (\Cref{ln:lfn:find-while-mark}) before it updates \code{pred} and \code{curr} 
(\Cref{ln:lfn:find-set-pred,ln:lfn:find-set-curr}). (Recall that the {\tref} and {\tm} fields are read in one atomic action).


\subparagraph*{Verifying linearizability of \code{contain}}
We use our framework to verify the linearizability of \code{contain} by
defining the notion of an order over memory locations, the notion of \emph{valid search path} for
key $k$ that starts at the \emph{head} node, and proving that the code respect the acyclically and preservation conditions.

As in our running example, we define the order over memory locations based on reachability. We say that there is a valid search path to a location $\loc_x$ for key $k$ from the head of the list, denoted by
$\lflQReachXK{\loc_x}{k}$,
if  $\loc_x$ is reachable from the head node to $\loc_x$ and either 
$x.\code{key}\leq k$ or $x$ is a marked node and its \tref-predecessor is on valid search path to $k$. 
Formally, search paths are defined as follows:
$$
\begin{array}{l}
\lflQReachXYK{\loc_r}{\loc_x}{k}
\eqdef
\exists \loc_0,\ldots,\loc_m.\,
\loc_0=\loc_r \land \loc_m=\loc_x \land {}
\\[2pt]
\qquad
\forall i=1..m.\, \loc_{i-1}.\tmnext.\tref=\loc_i \land (\loc_{i-1}.\code{key} \leq k  \lor \loc_{i-1}.\tmnext.\tm)

% \forall i=1..m.\, \loc_{i-1}.\code{key} < k \land \loc_{i-1}.\tmnext.\tref=\loc_i \land (\loc_{i}.\code{key} \leq k  \lor \loc_{i}.\tmnext.\tm)
% \QReachXK{x}{k}
% \eqdef
% \exists v_0,\ldots,v_m.\,
% v_0=\rootobj \land v_m=x \land
% \forall i=1..m.\, \child(v_{i-1},k,v_i)\ , \\
% \qquad \text{where} \ \child(v_{i-1},k,v_i) = (v_{i-1}.key < k \land v_{i-1}.\ileft = v_i) \lor (v_{i-1}.key > k \land v_{i-1}.\iright = v_i) \ .
\end{array}
$$
Note that a search path to $k$ might go through nodes with a key greater than $k$, but these nodes must be marked.

The acyclicity of the order stems from the immutability of keys and  invariant $I_{<}$ which ensures that cycles are impossible.

To prove the preservation of search paths to locations of modification it suffices to note that as marked nodes are never modified, it suffices to show the property hold for unmarked ones.
Note that marking a node increases the number of search path that goes through it.
Removing a marked node or adding a new ones does not  affect the search paths through the modified link.

To verify the linearizability of \code{contain} we 
establish the loop invariant in \Cref{ln:lfl:contains:inv} using the extension of our framework discussed in \Cref{rem:ReachWithField}.
This invariant, together with the definition of a search path ensures that as we get out of the loop only if we reached an unmarked node with the key that we look for, and in this case \code{marked} is false, or  
that during the traversal we never encountered that key that we look for or that this key was in a marked node. In either cases, the return value correspond to the contents of the abstract set at that time.


 
\begin{remarknum}\label{rem:ReachWithField}
We note that we can simplify the condition of the \code{while} loop in \code{contain} (\Cref{ln:lfl:contains:while}) to be \code{curr.key < key)} and still be able to verify the linearizability of \code{contain}.
Furthermore, we could have the current code as well as the simplified code using a simpler definition of a search path as well as a simpler the following definition of valid search paths which  does not depend on the values of {\tm}.
Namely, we could have defined  a valid search path to a location $\loc_x$ for key $k$ to be:
$$
\begin{array}{l}
\lflQReachXYK{\loc_r}{\loc_x}{k}
\eqdef
\exists \loc_0,\ldots,\loc_m.\,
\loc_0=\loc_r \land \loc_m=\loc_x \land {}
\\[2pt]
\qquad
\forall i=1..m.\, \loc_{i-1}.\tmnext.\tref=\loc_i \land \loc_{i-1}.\code{key} \leq k

% \forall i=1..m.\, \loc_{i-1}.\code{key} < k \land \loc_{i-1}.\tmnext.\tref=\loc_i \land (\loc_{i}.\code{key} \leq k  \lor \loc_{i}.\tmnext.\tm)
% \QReachXK{x}{k}
% \eqdef
% \exists v_0,\ldots,v_m.\,
% v_0=\rootobj \land v_m=x \land
% \forall i=1..m.\, \child(v_{i-1},k,v_i)\ , \\
% \qquad \text{where} \ \child(v_{i-1},k,v_i) = (v_{i-1}.key < k \land v_{i-1}.\ileft = v_i) \lor (v_{i-1}.key > k \land v_{i-1}.\iright = v_i) \ .
\end{array}
$$
We chose to present the more complicated code as it is the ones used in the skiplist algorithm discussed in the following section.
\end{remarknum}


==> notations.tex <==
%!TEX root=./main.tex

\section{Notations}\label{Se:Notations}


We denote by $\_$ an immaterial value which is implicitly existentially quantified.
We denote by $\bot$ the \emph{undefined} value. 
%
We write $\uplus$ to denote the union of  disjoint sets.
%
We denote the set of finite subsets of a set $X$ by $\psetfin X$.
%
We use $\partialto$ and $\totalto$ to denote \emph{partial} and \emph{total} functions, respectively.
%
%Given a function $f:A \partialto B$, we denote the \emph{domain} (or \emph{support}) and \emph{image} of $f$ by $\domof{f} = \{ a\in A \mid f(a) \neq  \bot\}$ and $\imageof{f} = \{ f(a) \in B \mid a \in A\}$, respectively.
Given a function $f:A \partialto B$, we refer to $A$ and $B$ as the \emph{domain} and \emph{codomain} of $f$, and denote them by $\domof{f}=A$ and $\codomof{f}=B$, respectively. We refer to the subset of $A$ on which $f$ is defined as the \emph{domain of definition} (or \emph{support}) of $A$, and denote it by $\supportof{f}= \{ a\in A \mid f(a) \in B\}$. We refer to the subset of $B$ onto which $f$ maps the elements  of $\supportof{f}$ as the \emph{range} (or \emph{image}) of $f$, and denote it by $\imageof{f} = \{ f(a)  \mid a \in \supportof{f}\}$, respectively.
%
We write $\totalto_{\fin}$ \resp. $\partialto_{\fin}$ to denote that a total \resp. partial function has a finite support.
%
By abuse of notation, we use $\bot$ to also denote any function with an empty support.
%
\ignore{
We denote 
the set of \emph{finite sequences} over a set $A$ by $\seq{A}$,
the empty sequence by $\emptyseq$, 
and the concatenation of sequences $F$ and $G$ by $F \cdot G$.
We write a sequence of $n$ elements by $\seqA{a_1,\ldots,a_n}$.
By abuse of notation, we sometimes treat a single element $x$ as the sequence  $\seqA x$.
%
Let $f:A \partialto B$ be a partial function from $A$ to $B$   and $F \in \seq{A \partialto B}$ be a sequence of such functions.
The \emph{overwrite} of $F$ by $f$, denoted by $\overwriteby{F}{f}$,
is
\[
        \overwrite{F}{f} \eqdef \lambda a \in A.\,
        \begin{cases}
                f(a) & f(a) \neq \bot \text{ or } F = \emptyseq\\
                (\overwrite{G}{g})(a) & f(a) = \bot \text{ and } F = G \cdot g \,. 
        \end{cases}
\]
Given functions $f,g:A \partialto B$, we write $f[g]$ as a shorthand for $\overwriteby{\seqA{f}}{g}$.
}
We denote by $f|_S$ the \emph{restriction} of function $f$ to $S$, i.e., $f|_S=\lambda x.\,\text{\it if}\,\,x\in S\text\,{\it then }\, f(x)\, \text{\it else } \bot$.



==> running-vs-cf.tex <==
\section{Notes on the Running Example}
The example of \Cref{Fi:Running} differs from the original contention-friendly tree~\cite{EuroPar13:CFTree,PFL16:CFTree} in a few points.
The most notable difference is that our traversals do not consult the \code{rem} flag, and in particular we do not need to distinguish between a left and right rotate, making the traversals' logic simpler. Proving the correctness of the algorithm with such traversals requires an \emph{unfixed} linearzation point. For our framework, the necessity to use an unfixed linearization point incurs no additional complexity.

The original algorithm performs backtracking by setting pointers from child to parent when nodes are removed. Instead, we restart the operation. This backtracking violates order requirements, and is left for future work.

Lastly, we fix a small bug in the description of~\cite{PFL16:CFTree}, where the \code{del} field was omitted in copying a rotated node.


%a. Our locate() doesn't check the removed flag (and doesn't care whether this is by a left or right rotation)
%
%      b. We don't perform backtracking when arriving to a removed node, they implement this by pointing to the parent and we don't modify these pointers on remove
%      
%      c. We copy also the del flag on rotate.
